S$^2$DN: Learning to Denoise Unconvincing Knowledge for Inductive Knowledge Graph Completion

Inductive Knowledge Graph Completion (KGC) aims to infer missing facts between newly emerged entities within knowledge graphs (KGs), posing a significant challenge. While recent studies have shown promising results in inferring such entities through knowledge subgraph reasoning, they suffer from (i) the semantic inconsistencies of similar relations, and (ii) noisy interactions inherent in KGs due to the presence of unconvincing knowledge for emerging entities. To address these challenges, we propose a Semantic Structure-aware Denoising Network (S$^2$DN) for inductive KGC. Our goal is to learn adaptable general semantics and reliable structures to distill consistent semantic knowledge while preserving reliable interactions within KGs. Specifically, we introduce a semantic smoothing module over the enclosing subgraphs to retain the universal semantic knowledge of relations. We incorporate a structure refining module to filter out unreliable interactions and offer additional knowledge, retaining robust structure surrounding target links. Extensive experiments conducted on three benchmark KGs demonstrate that S$^2$DN surpasses the performance of state-of-the-art models. These results demonstrate the effectiveness of S$^2$DN in preserving semantic consistency and enhancing the robustness of filtering out unreliable interactions in contaminated KGs.

==> checklist.tex <==
\section{Reproducibility Checklist}
This paper
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced [\textbf{yes}]
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results [\textbf{yes}]
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper [\textbf{yes}]
\end{itemize}
Does this paper make theoretical contributions? [\textbf{yes}]

\noindent If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. [\textbf{no}] We experimentally prove novel claims rather than theorem statements.
    \item All novel claims are stated formally (e.g., in theorem statements). [\textbf{partial}]
    \item Proof sketches or intuitions are given for complex and/or novel results. [\textbf{yes}]
    \item Appropriate citations to theoretical tools used are given. [\textbf{yes}]
    \item All theoretical claims are demonstrated empirically to hold. [\textbf{yes}]
    \item All experimental code used to eliminate or disprove claims is included. [\textbf{no}]
\end{itemize}
Does this paper rely on one or more datasets? [\textbf{yes}]

\noindent If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets [\textbf{yes}]
    \item All novel datasets introduced in this paper are included in a data appendix. [\textbf{NA}]
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. [\textbf{NA}]
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. [\textbf{yes}]
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. [\textbf{yes}]
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. [\textbf{NA}]
\end{itemize}
Does this paper include computational experiments? [\textbf{yes}]

\noindent If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. [\textbf{yes}].
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. [\textbf{yes}]
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. [\textbf{yes}]
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from [\textbf{yes}]
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. [\textbf{yes}]
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. [\textbf{yes}]
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. [\textbf{yes}]
    \item This paper states the number of algorithm runs used to compute each reported result. [\textbf{yes}]
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. [\textbf{yes}]
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). [\textbf{Partial}]
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. [\textbf{yes}]
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. [\textbf{yes}]
\end{itemize}

